Efficient Maintenance of Distance Labelling for Incremental Updates in Large Dynamic Graphs

Finding the shortest path distance between an arbitrary pair of vertices is a fundamental problem in graph theory. A tremendous amount of research has been successfully attempted on this problem, most of which is limited to static graphs. Due to the dynamic nature of real-world networks, there is a pressing need to address this problem for dynamic networks undergoing changes. In this paper, we propose an \emph{online incremental} method to efficiently answer distance queries over very large dynamic graphs. Our proposed method incorporates incremental update operations, i.e. edge and vertex additions, into a highly scalable framework of answering distance queries. We theoretically prove the correctness of our method and the preservation of labelling minimality. We have also conducted extensive experiments on 12 large real-world networks to empirically verify the efficiency, scalability, and robustness of our method.

==> section_Framework.tex <==
\section{Fully Dynamic Framework}
In this section, we propose a fully dynamic framework for distance queries on large-scale graphs. Within this framework, we develop a dynamic \emph{decremental algorithm}, which can efficiently update a highway cover labelling after an edge deletion, respectively.  

\subsection{Jumped-and-Pruned Searches}
To efficiently reflect changes on graphs, we develop a jumped-and-pruned search strategy for updating distance labelling. This requires us to identify two special types of vertices in a fully dynamic graph: \emph{affected vertices} and \emph{anchor vertices}. 

\subsubsection{Affected Vertices}\label{subsubsection:affected-vertices}
When an update operation occurs on a graph $G=(V,E)$, no matter whether it is an edge insertion or an edge deletion, there always exists a subset of ``affected'' vertices in $V$ whose labels need to be updated as a consequence of this update operation on the graph.  


\begin{definition}[affected vertex]\label{def:affected_vertex}
A vertex $v\in V$ is \emph{affected} by $G \hookrightarrow G'$ if $P_{G}(v, r)\not=P_{G'}(v,r)$ holds for at least one $r\in R$, and \emph{unaffected} otherwise.
\end{definition}

For simplicity, we use $\Lambda_r=\{v\in V|P_{G}(v, r)\not=P_{G'}(v,r)\}$ to denote the set of all affected vertices w.r.t. a landmark $r$ and $\Lambda=\bigcup_{r\in R}\Lambda_r$ refers to the set of all affected vertices.

\begin{example}
Consider Figure~\ref{fig:affected_vertices_example}(a) in which $0$ and $10$ are two landmarks. After inserting an edge $(2,5)$ in Figure~\ref{fig:affected_vertices_example}(b)-(c), we have the set of affected vertices $ \Lambda=\{0, 1, 2, 3, 5, 8, 9, 10, 13, 14\}$ because the edge $(2,5)$ lies in one of their shortest paths to $\{0, 10\}$, i.e., $\Lambda_0=\{5, 8, 9, 10, 13, 14\}$ and $\Lambda_{10}=\{0, 1, 2, 3\}$ are the set of affected vertices w.r.t $0$ and $10$, respectively. 

\begin{figure}[ht!]
\centering
\includegraphics[scale=0.5]{aff_vs_exmp.pdf}
\caption{An illustration of affected vertices by an edge insertion (2,5): (a) two landmarks $0$ and $10$ are highlighted in red; (b)-(c) affected vertices w.r.t. the landmarks $0$ and $10$ are highlighted in green, respectively.}
\label{fig:affected_vertices_example}
\end{figure}
\end{example}

The following lemma states how affected vertices relate to an edge being inserted or deleted.

\begin{lemma}\label{lemma:aff_vs_insertion}
When $G \hookrightarrow G'$ for an edge insertion, a vertex $v\in \Lambda_r$ iff there exists a shortest path between $v$ and $r$ in $G'$ that passes through the inserted edge $(a, b)$. Similarly, when $G\hookrightarrow G'$ for an edge deletion, a vertex $v\in \Lambda_r$ iff there exists a shortest path between $v$ and $r$ in $G$ that passes through the deleted edge $(a, b)$. 
\end{lemma}

Following Lemma \ref{lemma:aff_vs_insertion}, we have the following corollary.

\begin{corollary}\label{same_distance}
Let $r\in R$ be a landmark. When $G \hookrightarrow G'$, if $d_{G}(r,a) = d_{G}(r,b)$ holds, then we have $\Lambda_r=\emptyset$.% Similarly, when $G' \hookrightarrow G$, if $d_{G'}(r,a) = d_{G'}(r,b)$ holds, then we have $\Lambda(r)=\emptyset$.
\end{corollary}

This corollary allows us to reduce the search space for identifying affected vertices by considering only landmarks whose distances to $a$ and $b$ are different in an original graph. Without loss of generality, we assume that $d_G(r, b) > d_G(r, a)$ w.r.t. a landmark $r$ in the rest of this section. By Fact \ref{fact-deletion} and Lemma \ref{lemma:aff_vs_insertion}, we also have the following lemma.
 
\begin{lemma}\label{traverse-identifying-affected}
When $G \hookrightarrow G'$ with an inserted or deleted edge $(a,b)$, $d_G(v,r) \geq d_G(a,r)+1$ hold for any affected vertex $v\in \Lambda_r$.
\end{lemma}
\begin{proof} 
By Lemma \ref{lemma:aff_vs_insertion}, there exists a shortest path from any affected vertex $v$ to $r$ going through the affected edge $(a, b)$ and thus through $a$. Since $a$ is unaffected and the distance from $a$ to $v$ is equal to or greater than 1, $d_G(v, r) \geq d_G(a, r) + 1$ thus holds.
\end{proof}

Based on Lemmata \ref{lemma:aff_vs_insertion} and \ref{traverse-identifying-affected}, we can further reduce the search space of identifying affected vertices (will be further discussed in Section \ref{subsubsection:js-bfs}). 

\subsubsection{Anchor Vertices}\label{subsubsection:anchor-vertices}
While efficiently identifying affected vertices is critical for dynamic algorithms, it is equally important to efficiently update the labels of affected vertices against changes on a graph, without incurring unnecessary
searches. A natural thought is to naively run a full BFS from each landmark $r$ on the changed graph in order to decide the new distances of affected vertices w.r.t. $r$. However, this naive solution is inefficient, particularly when only a very small portion of vertices in a graph is affected by an update operation. Can we pinpoint the differences between the old labels of affected vertices in an original graph and their new labels in the changed graph, so as to change a distance labelling in an efficient way? 

To answer this question, we need to identify a special kind of affected vertices that have the smallest distance to a landmark $r$ on the changed graph among all affected vertices, which we call \emph{anchor vertices}. 

\begin{definition}[anchor vertex]\label{def:anchor_vertex}
When $G \hookrightarrow G'$, a vertex $v\in V$ is an \emph{anchor vertex} w.r.t. a landmark $r$ in $G'$ if $v\in \Lambda_r$ and  $d_{G'}(r, v)\leq d_{G'}(r, u)$ for any vertex $u\in \Lambda_r$.
\end{definition}

The following lemma states that the exact distances of anchor vertices can be inferred from their unaffected neighbours. Note that this does not generally hold for any affected vertices. Let $d^{*}_{G'}(r,v)$ refer to a \emph{contingent distance} between a landmark $r$ and a vertex $v\in \Lambda_r$ in $G'$, which is the minimum length of paths between $v$ and $r$ that go through only unaffected vertices in $G'$.


\begin{lemma}\label{lemma-inferred-vertices}
When $G \hookrightarrow G'$, if a vertex $v\in \Lambda_r$ has the smallest contingent distance to a landmark $r$ among all vertices in $ \Lambda_r$, then $v$ is an anchor vertex w.r.t. $r$ and $d_{G'}(r,v)=d^{*}_{G'}(r,v)$ holds.
\end{lemma}
\begin{proof}
    We prove this by contradiction. Assume that $d_{G'}(r,v)\neq d^{*}_{G'}(r,v)$. Since $d^{*}_G(v,r)$ is the minimum length of all paths between $v$ and $r$ that go through only unaffected vertices, it means that $d_G(r,v)< d^{*}_G(r,v)$ and one shortest path between $v$ and $r$ must go through at least one affected vertex $v'\in\Lambda_r$. Then $d^{*}_{G'}(v,r)>d^{*}_{G'}(v',r)$ must hold. This contradicts with the assumption that $v$ has the minimum contingent distance to $r$ in $\Lambda_r$ and thus $d_{G'}(r,v)=d^{*}_{G'}(r,v)$. Accordingly, $v$ must be an anchor vertex w.r.t. $r$. 
\end{proof}

Our observation is that, once anchor vertices are identified, we can locally infer their new distances from their unaffected neighbours. Then, 
new distances of other affected vertices can be inferred inductively by a level-by-level propagation in a BFS tree through unaffected neighbours and affected vertices whose new distances have already been inferred. 

\subsubsection{Jumped-and-Pruned BFS}\label{subsubsection:js-bfs}
Our decremental algorithm uses a \emph{jumped-and-pruned} search strategy to efficiently update a distance labelling. The key idea is that, instead of conducting a full BFS from a landmark to all vertices, we conduct a partial BFS (named as JP-BFS) that jumps from the root of a BFS directly to affected vertices, while unaffected vertices are skipped. Further, it prunes affected vertices after the jump. 

\begin{definition}
When $G \hookrightarrow G'$, 
a vertex $v$ is \emph{prunable} w.r.t. a landmark $r$ iff there exists a landmark $r'\in R-\{r\}$ such that all of the following conditions hold: 
\begin{itemize}
\item[(1)] $d_G(r, v)=d_G(r,r')+d_G(r',v)$; 
\item[(2)] $d_{G'}(r, v)=d_{G'}(r,r')+d_{G'}(r',v)$;
\item[(3)] $d_{G}(r',v)=d_{G'}(r',v)$.
\end{itemize}
\end{definition}

Intuitively, the conditions in the above definition state that we can prune a vertex $v$ only if there is another landmark $r'$ lying in the shortest path between this vertex and the landmark $r$ in both $G$ and $G'$, i.e. (1) and (2), and the distance from this vertex to $r'$ also remains the same in both $G$ and $G'$, i.e. (3). Since the labels of $v$ w.r.t. $r$ remain the same in $G$ and $G'$, a JP-BFS can thus prune $v$ and its child vertices from search. We will discuss these further in \ref{subsection:deletion}.

In a nutshell, a JP-BFS has the following two features:

\begin{itemize}
\item \textbf{Jumping} from the root to affected vertices to traverse through their neighbours in a localized fashion. 
\item \textbf{Pruning} affected vertices that are prunable whenever possible.
\end{itemize}

In the most general case, two kinds of JP-BFS may be needed. One kind of JP-BFS is to \emph{identify affected vertices w.r.t. a landmark $r$}. By Lemmata \ref{lemma:aff_vs_insertion} and \ref{traverse-identifying-affected}, such a JP-BFS jumps from the root $r$ to the vertex $b$, and starts to identify affected vertices iteratively through checking neighbours and their old distances. The other kind of JP-BFS is to \emph{update affected vertices w.r.t. a landmark $r$}. By Lemma \ref{lemma-inferred-vertices}, such a JP-BFS jumps from the root $r$ to anchor vertices, and starts to update the labels of affected vertices through a level-by-level propagation to 
infer their new distances.

In the following, we will discuss how these two kinds of JP-BFS are conducted and how prunable vertices are handled in our \emph{decremental algorithm}.
